Unsupervised Natural Language Inference Using PHL Triplet Generation

Transformer-based models achieve impressive performance on numerous Natural Language Inference (NLI) benchmarks when trained on respective training datasets. However, in certain cases, training samples may not be available or collecting them could be time-consuming and resource-intensive. In this work, we address the above challenge and present an explorative study on unsupervised NLI, a paradigm in which no human-annotated training samples are available. We investigate it under three settings: PH, P, and NPH that differ in the extent of unlabeled data available for learning. As a solution, we propose a procedural data generation approach that leverages a set of sentence transformations to collect PHL (Premise, Hypothesis, Label) triplets for training NLI models, bypassing the need for human-annotated training data. Comprehensive experiments with several NLI datasets show that the proposed approach results in accuracies of up to 66.75%, 65.9%, 65.39% in PH, P, and NPH settings respectively, outperforming all existing unsupervised baselines. Furthermore, fine-tuning our model with as little as ~0.1% of the human-annotated training dataset (500 instances) leads to 12.2% higher accuracy than the model trained from scratch on the same 500 instances. Supported by this superior performance, we conclude with a recommendation for collecting high-quality task-specific data.

==> tables/examples/nli.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{@{}p{0.36\linewidth}p{0.36\linewidth}c@{}}
        \toprule
        \textbf{Premise (P)} & \textbf{Hypothesis (H)} & \textbf{Label (L)}\\
        \midrule
        \textit{A football game with many males playing}  &  \textit{Some men are playing a sport} & Entails\\ 
        \textit{A man is riding the bike on highway.} & \textit{The man is sleeping in his room} & Contradicts\\
        \textit{A woman is talking on a cellphone.} & \textit{The woman is calling her mother} & Neutral \\
        \bottomrule 
    \end{tabular}
    \caption{Illustrative NLI examples for Entailment, Contradiction, and Neutral.}
    \label{tab:nli_examples}
\end{table}

==> tables/results/bias.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{ccp{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}}
        \toprule
        \textbf{Setting} & \textbf{Input} & \textbf{SNLI}  & \textbf{MNLI mat.} &  \textbf{MNLI mis.}  & \textbf{DNLI}\\
        \midrule
        % Expected & - & 33.33 & 33.33 & 33.33 & 33.33  \\
        % \midrule
        % NPH
        \multirow{2}{*}{NPH} & P Only & 33.00 & 34.57 & 34.34 & 34.76  \\
        & H Only & 36.05 & 32.39 & 32.88 & 30.69  \\
        \midrule
        % P
        \multirow{2}{*}{P} & P Only & 33.65 & 35.5 &	35.24 &	32.85  \\
        & H Only & 38.15 & 34.78 & 35.08 & 31.33  \\
        %PH
        \midrule
        \multirow{2}{*}{PH} & P Only & 33.12 & 34.01&	33.57 &	32.23 \\
        & H Only & 37.73 & 34.87&	35.67 & 32.79\\
    \bottomrule
    \end{tabular}
    \caption{Bias investigation for each setting, when only partial inputs (P-Only, H-Only) are given as input at inference time. Performance close to the random accuracy of $33.33\%$ is preferred.}
    \label{tab:robustness_baselines}
\end{table}

==> tables/results/few_shot.tex <==
\begin{table*}[t]
    \centering
    \small
    \resizebox{\linewidth}{!}{
    
    \begin{tabular}{ccccccc}
    % \begin{tabular}{p{0.8cm}p{2cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}}
    \toprule
        \textbf{Dataset} & \centering \textbf{Method} & \textbf{100} & \textbf{200} & \textbf{500} & \textbf{1000} & \textbf{2000}  \\
        \midrule
        % \midrule
        \multirow{3}{*}{SNLI}
        & From scratch & 44.62/37.36 &	48.97/34.71 &	58.54/44.01 &	65.36/37.24 &	72.51/45.59 \\
        
        & NPH Model & \textbf{64.82/49.72} &	\textbf{65.06/50.48} &	\textbf{66.97/52.33} &	\textbf{70.61/56.75} &	\textbf{73.7/59.0} \\
        & Adversarial*  & \textbf{-} &	\textbf{-} &	\textbf{70.85} &	\textbf{73.62} &	\textbf{74.31} \\
        
        \midrule
        \multirow{3}{*}{MNLI}
        & From scratch & 36.01/35.12 &	36.58/35.14 &	47.1/46.16 &	56.21/47.64 &	63.3/53.68 \\
        & NPH Model & \textbf{52.85/63.87} &	\textbf{53.61/63.87} &	\textbf{57.47/64.23} &	\textbf{60.42/65.62} &	\textbf{62.89/66.87} \\
        & Adversarial* & \textbf{-} &	\textbf{-} &	\textbf{-} &	\textbf{-} &	- \\
        
        % \midrule
        % \multirow{2}{*}{DNLI}
        % & From scratch & 42.22 &	71.19 &	75.47 &	79.28 & 85.23 \\
        % & NPH Model & 56.89 & 68.44 & 74.55 & 77.77 & 82.66 \\
        
        
        
        
    \bottomrule
    \end{tabular}
    }
    \caption{Demonstrating benefit of the model trained with procedurally generated PHL triplets in low-data regimes. Further fine-tuning our NPH model with the provided labeled instances achieves higher performance than the models fine-tuned from scratch. 
    Adversarial method corresponds to training a model from scratch with our procedurally generated PHL triplets and adversarially selected instances from the training dataset of SNLI/MNLI. * indicates that different labeled instances have been selected in this method that the other two methods.
    }
    \label{tab:few_shot_results}
\end{table*}

==> tables/results/perf.tex <==
\begin{table}[t]
    % \centering
    \small 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{p{0.4cm}p{2cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}}
    \toprule
        \textbf{Setting} &\centering\textbf{Model} & \textbf{SNLI}  & \textbf{MNLI mat.} &  \textbf{MNLI mis.}  & \textbf{DNLI} & \textbf{BNLI}\\
        \midrule
        % Sup. & - & 89.37 & 83.91 & 84.1 & 88.39 & -  \\

        % \midrule
        
        \multirow{5}{*}{NPH}
        % \cline{2-7}
        & $\mathcal{T}(\mathcal{P}(\text{C}))$ & 63.69 & \textbf{47.8} & \textbf{48.42} & \textbf{51.59} & \textbf{82.42} \\
        
        & $\mathcal{T}(\mathcal{P}(\text{R}))$  & 59.14 & 43.74 & 43.98 & 47.88 & 70.58 \\
        
        &$\mathcal{T}(\mathcal{P}(\text{W}))$ & 54.82 & 44.48 & 45.15 & 46.68 & 65.37 \\
        & $\mathcal{T}(\mathcal{P}(\text{C+R}))$ & \textbf{64.89} & 46.03 & 46.88 & 44.91 & 77.58 \\
        & $\mathcal{T}(\mathcal{P}(\text{C+R+W}))$ & 61.48 & 46.13 & 46.89 & 45.43 & 80.32 \\
        \midrule
        
        \multirow{8}{*}{P}
        & BERT & 35.09* & - & - & - & -\\
        & LXMERT & 39.03* & - & - & -& - \\
        & VilBert & 43.13* & - & - & - & -\\
        & MACD+COCO & 52.63* & - & - & - & - \\
        & MACD+Flickr30k & 52.27* & - & - & - & - \\
        % \cline{2-7}
        % \midrule
        
        % P & $\mathcal{T}(\text{SNLI})$ & 65.72 & 49.56 & 50.00 & 43.27 & 67.78\\
        & $\mathcal{T}(\text{SNLI})$ & 65.72 & 49.56 & 50.00 & 43.27 & 67.78\\
        
        % P & \quad{+}$\mathcal{T}(\mathcal{P}(\text{C}))$ & 65.36 & 49.91 & 49.24 & 46.25 & 70.07\\
        % P & \quad{+}$\mathcal{T}(\mathcal{P}(\text{R}))$ & \textbf{65.90} & 48.53 & 48.36 & 44.97 & 66.43\\
        & \quad{+}$\mathcal{T}(\mathcal{P}(\text{C}))$ & 65.36 & 49.91 & 49.24 & 46.25 & 70.07\\
        & \quad{+}$\mathcal{T}(\mathcal{P}(\text{R}))$ & \textbf{65.90} & 48.53 & 48.36 & 44.97 & 66.43\\
        
        
        \midrule
        
        \multirow{3}{*}{PH}
        & MaxProbFilt & 66.67 & 53.37 & 55.17 & - & -\\
        & \quad{+}$\mathcal{T}(P)$ & 66.75 & 50.22 & 50.37 & - & -\\
        & \quad{+}P-Model & 65.60 & 52.97 & 53.44 & - & -\\
        
        % SNLI
        % MNLI
        % DNLI

    \bottomrule
    \end{tabular}
    }
    \caption{Accuracy of models in the three unsupervised settings on various datasets. C, R, and W correspond to COCO, ROC, and Wiki respectively. Results marked with * have been taken from \cite{cui-etal-2020-unsupervised}.}
    \label{tab:perf_table}
\end{table}
